Performance Comparison of Graph Representations Which Support Dynamic Graph Updates

Research in graph-structured data has grown rapidly due to graphs' ability to represent complex real-world information and capture intricate relationships, particularly as many real-world graphs evolve dynamically through edge/vertex insertions and deletions. This has spurred interest in programming frameworks for managing, maintaining, and processing such dynamic graphs. In this report, we evaluate the performance of PetGraph (Rust), Stanford Network Analysis Platform (SNAP), SuiteSparse:GraphBLAS, cuGraph, Aspen, and our custom implementation in tasks including loading graphs from disk to memory, cloning loaded graphs, applying in-place edge deletions/insertions, and performing a simple iterative graph traversal algorithm. Our implementation demonstrates significant performance improvements: it outperforms PetGraph, SNAP, SuiteSparse:GraphBLAS, cuGraph, and Aspen by factors of 177x, 106x, 76x, 17x, and 3.3x in graph loading; 20x, 235x, 0.24x, 1.3x, and 0x in graph cloning; 141x/45x, 44x/25x, 13x/11x, 28x/34x, and 3.5x/2.2x in edge deletions/insertions; and 67x/63x, 86x/86x, 2.5x/2.6x, 0.25x/0.24x, and 1.3x/1.3x in traversal on updated graphs with deletions/insertions.

==> src/tab-compare.tex <==
\begin{table}[hbtp]
  \centering
  \caption{Speedup of our multicore implementation of Leiden algorithm compared to other state-of-the-art implementations. Direct comparisons entail running the given implementation on our servers, while indirect comparisons (marked with a $*$, explained in Section \ref{sec:comparison-indirect}) involve comparing results relative to a common reference\ignore{(original Leiden)}.\ignore{Notably, the Leiden implementations vary in their classification, with some being multi-core and others multi-node.}}
  \label{tab:compare}
  \begin{tabular}{|c|c||c|}
    \toprule
    \textbf{Leiden implementation} &
    \textbf{Parallelism} &
    \textbf{Our Speedup} \\
    \midrule
    Original Leiden \cite{com-traag19} & Sequential & $436\times$ \\ \hline
    igraph Leiden \cite{csardi2006igraph} & Sequential & $104\times$ \\ \hline
    NetworKit Leiden \cite{staudt2016networkit} & Parallel & $8.2\times$ \\ \hline
    cuGraph Leiden \cite{kang2023cugraph} & Parallel (GPU) & $3.0\times$ \\ \hline
    ParLeiden-S \cite{huparleiden} & Parallel & $18\times^*$ \\ \hline
    ParLeiden-D (8 nodes) \cite{huparleiden} & Multi-node & $22\times^*$ \\ \hline
  \bottomrule
  \end{tabular}
\end{table}

